Double-Loop Unadjusted Langevin Algorithm

A well-known first-order method for sampling from log-concave probability distributions is the Unadjusted Langevin Algorithm (ULA). This work proposes a new annealing step-size schedule for ULA, which allows to prove new convergence guarantees for sampling from a smooth log-concave distribution, which are not covered by existing state-of-the-art convergence guarantees. To establish this result, we derive a new theoretical bound that relates the Wasserstein distance to total variation distance between any two log-concave distributions that complements the reach of Talagrand T2 inequality. Moreover, applying this new step size schedule to an existing constrained sampling algorithm, we show state-of-the-art convergence rates for sampling from a constrained log-concave distribution, as well as improved dimension dependence.

==> sections/DL_ULA.tex <==
\section{Double Loop Unadjusted Langevin Algorithm}

In this section, we present a modified version of the standard ULA for sampling from an unconstrained distribution, that we will analyze in the following section. This modified version of ULA involves a new step size schedule as well as a projection step. We will show that it allows to obtain improved convergence rate, as well as the first convergence rate in $\W_2$-distance for overdamped Langevin dynamics.

We will then apply the same modification to an existing constrained sampling algorithm, and show that it allows both to obtain an asymptotic convergence and to improve the convergence rate.

\subsection{DL-ULA for unconstrained sampling}

We consider the problem of sampling  from a smooth and unconstrained probability measure $\mu^* \propto e^{-f(x)} \der x$, where $f:\R^d \rightarrow \R$ is differentiable. To this end, we apply the standard ULA in a double-loop fashion, and decrease the step size only between each inner loop. Moreover, each inner loop is followed by a projection step onto some Euclidean ball. The procedure is summarized in Algorithm~\ref{alg:DL_ULA}.

The projection step appears to be crucial in our analysis in order to control the tail of the sample distribution, which is necessary for bounding its Wasserstein distance to the target distribution. 

\begin{algorithm}[!t]
   \caption{Double-loop Unadjusted Langevin Algorithm (DL-ULA)}
   \label{alg:DL_ULA}
\begin{algorithmic}
\STATE \textbf{Input}: Smooth unconstrained probability measure $\mu^*$, step sizes $\{\gamma_k\}_{k\ge 1}$, number of (inner) iterations $\{n_k\}_{k\ge 1}$, initial probability measure ${\mu}_0$ on~$\R^d$, and thresholds $\{\tau_k\}_{k \ge 1}$.
\STATE \textbf{Initialization:} Draw a sample $x_0$ from the probability measure ${\mu}_{0}$.%, namely,  $\ol{x}_0 \sim {\ol{\mu}_0}$. 
\FOR{$k=1, \ldots$}
\STATE $x_{k,0} \leftarrow x_{k-1}$
\FOR{$n=1,\ldots,n_k$}
\STATE $x_{k,n+1} \leftarrow x_{k,n} - \gamma_k \nabla f(x_{k,n}) + \sqrt{2\gamma_k} g_{k,n}$, where $g_{k,n} \sim \mathcal{N}(0,I_d)$.
\ENDFOR
\STATE $x_{k} \leftarrow x_{k,i}$, where $i$ is drawn from the uniform distribution on $\{1,\cdots,n_k\}$.
\IF{$\|x_{k}\|_2 > \tau_k$}
\STATE $x_{k}\leftarrow \tau_k x_{k}/\| x_{k}\|_2$. 
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


%Although these little modifications...

\subsection{DL-MYULA for constrained sampling}

Consider sampling from a log-concave distribution over a convex set $\Omega \subset \R^d$, i.e.,
\begin{equation}
\mu^*(x)
= 
\begin{cases}
e^{-f(x)} / \int_\Omega e^{-f(x')}dx' & x\in \Omega \\
0 & x\notin \Omega.
\end{cases}
\label{eq:constrained-dist}
\end{equation}

In \cite{durmus2018efficient,brosse2017sampling}, the authors propose to reduce this problem to an unconstrained sampling problem by penalizing the domain outside $\Omega$ directly inside the probability measure using its Moreau-Yoshida envelop. More precisely, they propose to sample from the following unconstrained probability measure $\der \mu_\lam(x) \propto e^{-f_\lam(x)} \der x$ where $f_\lam:\R^d \rightarrow \R$ is defined as:
\begin{align}
f_\lam(x) = f(x) + \frac{1}{2\lam}\|x - \text{proj}_\Omega(x)\|_2^2,
\qquad \forall x\in \R^d,
\label{eq:penalized_dist}
\end{align}

where $\text{proj}_\Omega:\R^d \rightarrow \Omega$ is the standard projector operator onto $\Omega$ defined as $\text{proj}_\Omega(x) = \argmin_{y \in \Omega} \|x-y\|_2$. Note that this penalty is easily differentiable as soon as the projection onto $\Omega$ can be computed since $\nabla f_\lam(x) = \nabla f(x) + \frac{1}{\lam} (x - \text{proj}_\Omega(x))$.

By bounding the $\TV$ distance between $\mu_\lam$ and $\mu^*$, they showed that, by sampling from $\mu_\lam$ with $\lam$ small enough, it is possible to sample from $\mu^*$ with arbitrary precision. This algorithm is called Moreau-Yoshida ULA (MYULA).

Building on this approach, we can apply our double loop algorithm, modifying both the step size as well as the penalty parameter $\lam$ between each inner loop (Algorithm~\ref{alg:DL_MYULA}).

In addition to providing improved rate, as we will show later, our algorithm also has the advantage that it can use a decreasing penalty parameter $\lam$ so as to guarantee asymptotic convergence of the algorithm to the target distribution. On the other hand, MYULA uses constant penalty $\lam$, and thus saturates after a certain number of iterations.

\begin{algorithm}[h!]
   \caption{DL-MYULA}
   \label{alg:DL_MYULA}
\begin{algorithmic}
\STATE \textbf{Input}: Smooth constrained probability measure $\mu^*$, step sizes $\{\gamma_k\}_{k\ge 1}$, penalty parameters $\{\lam_k\}_{k\ge 1}$, number of (inner) iterations $\{n_k\}_{k\ge 1}$, initial probability measure ${\mu}_0$ on~$\R^d$, and thresholds $\{\tau_k\}_{k \ge 1}$.
\STATE \textbf{Initialization:} Draw a sample $x_0$ from the probability measure ${\mu}_{init}$.%, namely,  $\ol{x}_0 \sim {\ol{\mu}_0}$.
\FOR{$k=1, \ldots$}
\STATE $x_{k,0} \leftarrow x_{k-1}$
\FOR{$n=1,\ldots,n_k$}
\STATE $x_{k,n+1} \leftarrow x_{k,n} - \gamma_k (\nabla f(x_{k,n}) + \frac{1}{\lam_k} (x_{k,n} - \text{proj}_\Omega(x_{k,n}))) + \sqrt{2\gamma_k} g_{k,n}$, where $g_{k,n} \sim \mathcal{N}(0,I_d)$.
\ENDFOR
\STATE $x_{k} \leftarrow x_{k,i}$, where $i$ is drawn from the uniform distribution on $\{1,\cdots,n_k\}$.
\IF{$\|x_{k}\|_2 > \tau_k$}
\STATE $x_{k}\leftarrow \tau_k x_{k}/\| x_{k}\|_2$. 
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

%In \cite{brosse2017sampling}, the authors use a constant parameter $\lam$ 


%lambda fixed, variable penalty 



==> sections/convergence.tex <==
%!TEX root = ../dlula.tex

\section{Convergence analysis \label{sec:cvg}}

%For simplicity, we will assume that the target distribution $\mu^*$ and the smoothing distributions $\mu_\rho$ all have mean $0$.
In this section, we derive the convergence rate for Algorithms~\ref{alg:DL_ULA} and ~\ref{alg:DL_MYULA}. The global idea for showing the convergence of these algorithms is to use the inequality~\eqref{descent_lemma} recursively between each successive outer loop. We denote as $\bar{\mu}_k$ the average distribution associated to the iterates of outer iteration $k$ just \emph{before} the clipping step. Similarly, we denote as $\tilde{\mu}_k$ the same distribution \emph{after} the clipping step.

Each outer iteration $k$ uses as a starting point a sample from the previous outer iteration $x_{k,0} \sim \tilde{\mu}_{k-1}$. Therefore, we can apply the inequality~\eqref{descent_lemma} to the outer iteration $k$ to obtain
\begin{equation}
\KL(\bar{\mu}_k; \mu^*) \leq \frac{\W_2^2(\tilde{\mu}_{k-1}, \mu^*)}{2 \gamma_k n_k} + Ld\gamma_k.
\label{DL_descent_lemma}
\end{equation}

In order to unfold the recursion, we must have a bound on $\W_2^2(\tilde{\mu}_{k-1}, \mu^*)$ in terms of $\KL(\bar{\mu}_{k-1}, \mu^*)$. Using the light tail property of log-concave distributions, it is easy to obtain a bound between  $\W_2^2(\tilde{\mu}_{k-1}, \mu^*)$ and  $\W_2^2(\bar{\mu}_{k-1}, \mu^*)$. However, it is not clear how to bound  $\W_2^2(\bar{\mu}_{k-1}, \mu^*)$ by $\KL(\bar{\mu}_{k-1}, \mu^*)$.

As an intermediate step in the convergence analysis, we derive in the next section a bound  between the $\W_2$-distance and the $\TV$-distance between two general log-concave probability measures, which can then be extended to a $\W_2$-$\KL$ bound using Pinsker's inequality.


\subsection{Relation Between $\W_2$- and $\TV$-Distances}

%While it can be shown that log-concave distribution generally have rather light tail by definition, this assumption is still restrictive and does not hold for any unconstrained log-concave distribution. However, it still holds for interesting non-strongly log-concave distribution (e.g., $d\mu(x) \propto e^{-\|x\|_1}dx$), and it does trivially hold for any log-concave distribution constrained over a bounded set $\Omega$ containing $0$, in which case $\beta = \text{diam}(\Omega)$ and $\sigma = \sqrt{e}$ where $\text{diam}(\Omega)$ is the diameter of $\Omega$.

When  $\mu$ and $\nu$ are both compactly supported on an Euclidean ball of diameter $D$, then it is well-known that $\W_2(\mu,\nu) \leq D \sqrt{\|\mu-\nu\|_{\TV}}$~\cite{gibbs2002choosing}. Otherwise, if either $\mu$ or $\nu$ is not compactly supported, their fast-decaying tail (Lemma~\ref{lem:light_tail}) allows us to derive a similar bound, as summarized next and proved in Appendix~\ref{sec:WKLbound}.

%\subsection{Relaxed  transport inequality}
%
%A relation that will be recurrently used in the analysis is a bound between the 2-Wasserstein distance and the KL divergence of two log-concave measures defined on unbounded domains.
%
%A well known inequality between these two quantities is the transport inequality, which states that if $\mu$ is $\kappa$-strongly log concave, then $\frac{\kappa}{2}W_2^2(\mu, \nu) \leq KL(\nu || \mu)$ for all measure $\nu$ on $\R^d$ ~\cite{gozlan2010transport}.
%
%However, this inequality does not hold if $\mu$ is only log-concave. On the other hand, this inequality gives a bound on the Wasserstein distance between $\mu$ and any other measure $\nu$ (not necessarily log-concave). Instead, we provide the following bound, where both $\mu$ and $\nu$ are log-concave (but not necessarily strongly log-concave).
%
%To do so, we will use the fact that log-concave distributions necessarily have sub-exponential tail~\cite{cule2010theoretical}. \anote{Merged two cases in next lemma to one expression to later remove the assumption on R and for Corollary 5 to correctly hold.}
%\anote{Corrected the next lemma to hold for all R and added the exact constants. Matter of personal taste but I think the new proof is a bit more pro.}





%\anote{the previous choice of R below did not necessary meet the conditions of old lemma, which is corrected below.}
\begin{lem}\label{lem:cor-now-lem}
\textbf{\emph{($\W_2$-$\TV$ distances inequality)}}
Let $\mu,\nu$ be log-concave probability measures on $\R^d$ both satisfying Assumption~\ref{assumption:lighttail} with $(\eta, M_\eta)$. Then, for some scalar $c \in \R$,
%\begin{equation}
%\W_2^2(\mu, \nu) \leq 
%(2\sqrt{2}+26) \max\l( \b^2\log^2\l(\frac{1}{KL(\mu || \nu)} \r), \sigma^2 \log \l( \frac{1}{KL(\mu||\nu)}\r) , \b^2 ,\sigma^2 \r)
%\sqrt{KL(\mu||\nu)}.
%\end{equation}
\begin{equation}
\begin{split}
&\W_2(\mu, \nu) \leq cd\max\l(\log\l(\frac{1}{\|\mu - \nu\|_{\TV}}\r), 1\r) \sqrt{\| \mu-\nu\|_{\TV}}.
%\sqrt{\frac{2d^2}{\eta^2} + M_\eta} 
\end{split}
\label{eq:corr-result}
\end{equation}
\end{lem}

\noindent In a sense, \eqref{eq:corr-result} is an alternative to the powerful $T_2$ inequality which does not apply generally in our setting \cite{gozlan2010transport}. Indeed, for $C_\mu>0$, recall that a probability measure $\mu$ satisfies Talagrand's $T_2(C_\mu)$ transportation inequality if 
\begin{align}
\W_2(\mu, \nu) \leq C_\mu \sqrt{\KL(\mu ; \nu)},
\label{eq:T2-recall}
\end{align}
for  any probability measure $\nu$. Above, $C_\mu$ depends only on $\mu$ and, in particular, if $\mu$ is $\kappa$ strongly log-concave,\footnote{If $\der\mu \propto e^{-f}\der x$, then we say that $\mu$ is $\kappa$ is strongly log-concave if $f$ is $\kappa$ strongly convex. } then \eqref{eq:T2-recall} holds with $C_\mu=\mathcal{O}(1/\sqrt{\kappa})$~\cite{gozlan2010transport}. In this  work, the target measures that we consider are not necessarily strongly log-concave measures, leaving us in need for a replacement to \eqref{eq:T2-recall}. 
% and, as we will see shortly, the iterates of Algorithm~\ref{LC-LD} also do not follow strongly log-concave distributions. 
 In our analysis, \eqref{eq:corr-result} serves as a replacement for \eqref{eq:T2-recall}. Indeed, using the Pinsker's inequality \cite{pinsker1960information}, an immediate consequence of \eqref{eq:corr-result} is that
\begin{equation}
\W_2(\mu,\nu) = \wt{\mathcal{O}} (\KL(\mu;\nu)^{\frac{1}{4}} ). 
\label{eq:W2-KL-bound}
\end{equation}
%\begin{proof-sketch}
%The idea of the proof is to split the transportation cost between transport occurring inside and outside a ball of radius $R$. Inside this ball, we use an existing bound between the Wasserstein distance and the TV distance. Then, we use the sub-exponential properties of the distributions in order to bound the remaining transportation cost.
%\end{proof-sketch}

In fact, \eqref{eq:corr-result} might also be of interest in its own right, especially when working with non-strongly log-concave measures. For example, under the additional Assumption~\ref{assumption:lighttail}, it is easy to use \eqref{eq:W2-KL-bound} to extend the well-known $\mathcal{O}(\epsilon^{-2})$ convergence rate of ULA in KL divergence to a $\wt{\mathcal{O}}(\epsilon^{-8})$ convergence rate in $\W_2$ distance in the non-strongly log-concave setting. To the best of our knowledge, such a result does not exist in the literature. 


%\anote{Paul, could you add citation and correct the result below?}
\iffalse{
Indeed, the following result immediately follows by applying \eqref{eq:W2-KL-bound} to \cite[Corollary 7]{durmus2018analysis}. 
\begin{corr}
\label{cor:durmus-w-our-t2}
\emph{\textbf{(iteration complexity of ULA in $\W_2$)}}
Consider a probability measure $\mu^*$ in $\R^d$, such that $\der \mu^* \propto e^{-f} \der x$, where $f$ is convex and $\nabla f$ is $L$ Lipschitz continuous. 
%Assume $f$ is convex and $L$-Lipschitz gradient. Let $\epsilon > 0$ and $\mu_0$ be a probability measure on $\R^d$. 
Given a target accuracy of $\epsilon$, suppose we apply ULA in ~\eqref{Langevin_iter} with the initialization from $x_0 \sim {\mu}_0$ and the step size
\begin{align}
\gamma \leq \frac{1}{L} \min\l( \frac{\epsilon^4}{2d}, 1\r).
\end{align}
Let $\wh{\mu}_k$ denote the probability measure associated with the $k$-th iteration of ULA, namely, $x_k\sim \wh{\mu}_k$. 
After 
\begin{align}
n \geq \frac{\W_2^2(\wh{\mu}_0, \mu^*)}{\gamma \epsilon^4}
\end{align}
iterations, we reach  $\W_2(\bar{\mu}_{n}, \mu^*) \leq \epsilon$, where $\bar{\mu}_{n} = \frac{1}{n} \sum_{k=1}^{n} \wh{\mu}_k$ is the average of the probability measures up to the iteration $n$. 
\end{corr}
\fi

%
%Suppose that we want to sample from a smoothable distribution $\mu^*$ with smoothing family $\{\mu_k\}_k$.  
%In this section, we bound $\W_2(\bar{\mu}_k, \mu^*)$ where $\{\bar{\mu}_k\}_k$ is generated by Algorithm~\ref{LC-LD}, for some particular choice of sequences $\{\rho_k,n_k,\gamma_k\}_{k\ge 0}$. 
%

\begin{table*}[h!]
\centering
\hspace*{-5mm}
\begin{tabular}{|l||*{3}{c|}}\hline
%\backslashbox{Mask}{Decoder}
\makebox[4em]{\small Literature} &\makebox[4em]{$\W_2$}&\makebox[4em]{{$\TV$}}&\makebox[4em]{\small $\KL$}  \\\hline \hline
%\makecell{\cite{cheng2017convergence, durmus2018analysis, dalalyan2017user}} & {\small$\tilde{O}\l(Ld m^{-2}\epsilon^{-2} \r)$ } &  \small $\wt{O} \l(Ld m^{-2}\epsilon^{-2} \r)$ &  \small$\wt{O}\l( Ld m^{-2}\epsilon^{-1}  \r)$  \\\hline
\makecell{\cite{durmus2018analysis}} & - &  \small $\wt{O} \l(Ld^3\epsilon^{-4} \r)$ &  \small$\wt{O}\l(Ld^3\epsilon^{-2} \r)$  \\\hline
\makecell{\cite{durmus2017nonasymptotic}} & - &  \small $\wt{O} \l(L^2d^5\epsilon^{-2} \r)$ &  -   \\\hline
\makecell{\cite{zou2018stochastic}} & $\wt{O} \l(L^2 d^{10.5}\epsilon^{-6}\r)^*$ &  - &  -  \\\hline
\small Our work & \small $\wt{O} \l(Ld^8\epsilon^{-6}\r)$ &  \small $\wt{O} \l(Ld^2\epsilon^{-3} \r)$ &  \small$\wt{O}\l(Ld^2\epsilon^{-\frac{3}{2}} \r)$ \\\hline
\end{tabular}
\vspace{1mm}
\caption{Complexity of sampling from a smooth and log-concave probability distribution. For each metric, the entry corresponds to the total number of iterations to use in order to reach an $\epsilon$ accuracy in the specified metric. ($^*$ For comparison purpose, we extended the proof in \cite{zou2018stochastic} in the case where the distribution satisfies the weaker assumption~\ref{assumption:lighttail}. The dimension dependence is thus different from \cite{zou2018stochastic}).}
%\anote{Paul, I'm unfamiliar with the literature but I was expecting the strongly convex rates to be linear. What am I missing?}
\label{table:unconstrained}
\end{table*}

\subsection{Convergence Analysis of DL-ULA}

Having covered the necessary technical tools above, we now turn our attention to the convergence rate of Algorithm~\ref{alg:DL_ULA}. The final step to take care of is to choose the sequences $\{\gamma_k\}_{k\ge 1}$ and $\{n_k\}_{k\ge 1}$ so as to obtain the best possible convergence guarantees. We summarize our result in Theorem~\ref{thm:convergence_DL_ULA}.


\begin{thm} \label{thm:convergence_DL_ULA}
\textbf{\emph{(iteration complexity of DL-ULA)}}
Let $\mu^*$ be a $L$-smooth log-concave distribution satisfying assumption~\ref{assumption:lighttail}. Suppose that $\mu_0$ also satisfies assumption~\ref{assumption:lighttail}. 
For every $k\ge 1$, let
\begin{align}
n_k = L M d k^2e^{3k} % \approx_{\b,\s} \frac{d  e^{k(\frac{1}{2s}+3)} }{\W_2(\ol{\mu}_0,\mu^*)^{\frac{1}{s}+6}} ,
\end{align}
\begin{align}
\g_k = \frac{M}{Ld} e^{-2k} %\approx_{\b,\s} \frac{\W_2(\ol{\mu}_0,\mu^*)^{\frac{1}{s}+4}}{d e^{k(\frac{1}{2s}+2 )}},
\end{align}
\begin{align}
\tau_k = M k. % \gtrsim_{\b,\s}  \max\l(   \log^2\l( \frac{1}{\epsilon}\r), 1 \r),
\label{eq:thresh-req-thm}
\end{align}
where $M = \sqrt{\frac{2d(d+1)}{\eta^2} + M_\eta^2} = \mathcal{O}(d)$.

Let $\bar{\mu}_k, \tilde{\mu}_k$ be the average distributions associated with the iterates of outer iteration $k$ of DL-ULA using the parameters above, just before and after the clipping step respectively. Then, $\forall \epsilon > 0$, we have:
\begin{itemize}
\item After $N^{\KL} = \tilde{\mathcal{O}}(Ld^2\epsilon^{-\frac{3}{2}})$ total iterations, we obtain $\KL(\bar{\mu}_k; \mu^*) \leq \epsilon$.
\item After $N^{\TV} = \tilde{\mathcal{O}}(Ld^2\epsilon^{-3})$ total iterations, we obtain $\|\tilde{\mu}_k - \mu^*\|_{\TV} \leq \epsilon$. 
\item After $N^{\W_2} =  \tilde{\mathcal{O}}(Ld^8\epsilon^{-6})$ total iterations, we obtain $\W_2(\tilde{\mu}_k, \mu^*) \leq \epsilon$.
\end{itemize}
\end{thm}


\noindent A few remarks about Theorem \ref{thm:convergence_DL_ULA} are in order.

\paragraph{Geometric sequences.} Theorem \ref{thm:convergence_DL_ULA} prescribes a geometric sequence for the choice of $\{\gamma_k\}_k$ and $\{n_k\}_k$. As outer iteration counter $k$ increases, more and more ULA (inner) iterations are performed with the constant step-size $\gamma_k$. Asymptotically, we observe that the step size decreases at a rate $n^{-\frac{2}{3}}$ where $n$ is the total number of ULA iterations. This decaying rate is faster than the standard decaying rate of $n^{-\frac{1}{2}}$ for ULA ~\cite{durmus2018analysis}.

In constrast to convex optimization where a global optimum can be provably reached with constant step-size, ULA cannot converge to the target distribution $\mu^*$ when using non-zero step-size, since the stationary distribution of ULA iterates ~\eqref{Langevin_iter} when using a non-zero step size is different from the target distribution. Asymptotically, it is thus desirable to use as small a step-size as possible.

This double loop approach resembles the doubling trick in online learning ~\cite{rakhlin2013online}. However, in contrast with online learning where this does not affect the convergence rate, we prove that this procedure allows to improve the convergence rate of ULA.

%\paragraph{Benefit of outer loop.} 
%Note that the outer loop of Algorithm \ref{LC-LD} plays an important role in its computational efficiency. In principle, we can achieve the target accuracy of $\epsilon$ with a single application of ULA to sample from $\mu_{\rho_1}$ for a sufficiently large $\rho_1$, namely, by running one outer iteration of  Algorithm \ref{LC-LD}. There are two issues with this approach. First, in the case of non-smooth sampling, such an approach would require to use a very small step size even in the early iterations, leading to slow learning. Second, we will see in Example 1 in Section \ref{sec:examples} that HULA (with its variable step size in outer iterations) improves over standard ULA for sampling from smooth log-concave probability measures. Instead, with a small  outer of iterations (logarithmic in target accuracy), HULA has a course-to-fine hierarchy which provides both numerical stability and speed. The same attributes has led to the overwhelming success of smoothing techniques in convex optimization \cite{nesterov2005smooth}.
%\anote{is this reasonable? what can we add?} 

\paragraph{Thresholding.} Although the initial and target distributions are both log-concave, and thus have a sub-exponential tail, the sample distributions $\bar{\mu}_k$ are not generally log-concave, and it is not clear whether they also share the sub-exponential tail property. The clipping step at the end of each outer iteration provides a way to enforce the light tail property, so that we can still apply a bound similar to~\eqref{eq:corr-result}. This procedure is made clearer in the proof of the theorem.

This procedure also provides more stability in the early outer iterations where the step-size is the largest. Moreover, since $\lim_{k \rightarrow \infty} \tau_k = \infty$, the clipping step asymptotically never applies in practice.

%\paragraph{Convergence in $\KL$ divergence} After the clipping step, the clipped distribution . For this reason, we state the convergence rate in $\KL$ divergence using the distribution \emph{before} the clipping step, i.e., $\bar{\mu}_k$.

\paragraph{Convergence rate comparison} Table~\ref{table:unconstrained} summarizes various convergence rates of Langevin dynamics based methods applied to general log-concave distributions. We observe that DL-ULA achieves improved convergence rate either in terms of dimension or accuracy dependence. Compared to \cite{durmus2017nonasymptotic}, the convergence rate in $\TV$ distance is worse in terms of accuracy $\epsilon$ but enjoys much better dimension dependence, and is also better in terms of Lipschitz constant dependence.

 
%the normalization step in Algorithm~\ref{alg:DL_ULA} guarantees that the output measures has sufficiently light tails, as required in Assumption~\ref{assumption:lighttail}. In turn, Lemma \ref{lem:cor-now-lem} bounds $\W_2$ with $\TV$ and allows us to recursively bound the error of each outer iteration of Algorithm \ref{LC-LD} with the previous iteration. Without thresholding and in the absence of strong log-concavity, it is not clear to us whether the outputs of Algorithm~\ref{LC-LD} provably conserve a sufficiently light tail that would allow us to bound the $\W_2$ distance. The thresholding also introduces an exponentially small error into Algorithm \ref{LC-LD}. In practice, we found that the threshold could be set very large, so that the thresholding step in Algorithm~\ref{LC-LD} is never activated.
%\anote{Is this a reasonable argument? what can we add?} 



%\newpage
\subsection{Convergence rate of DL-MYULA}

We now analyze the convergence of DL-MYULA. In Algorithm~\ref{alg:DL_MYULA}, both the step-size and the penalty parameter $\lam$ are decreased after each outer iteration. Therefore, at each outer iteration $k$, we aim to sample from the unconstrained penalized distribution $\der \mu_{\lam_k} \propto e^{-f_{\lam_k}(x)} \der x$ as defined in equation~\eqref{eq:penalized_dist}. 

Similarly as previously, we will use Lemma~\ref{descent_lemma} after each outer iteration. However, since the target distribution of outer iteration is $\mu_{\lam_k}$ instead of $\mu^*$, the inequality reads as follows:
\[
\KL(\bar{\mu}_k; \mu_{\lam_k}) \leq \frac{\W_2^2(\tilde{\mu}_{k-1}, \mu_{\lam_k})}{2 \gamma_k n_k} + Ld\gamma_k.
\]
where we recall that $\bar{\mu}_k$ is the average iterate distribution of outer iteration $k$ just before the clipping step, and $\tilde{\mu}_k$ is the one just after the clipping step.

In order to use a similar recursion argument as previously, we must thus bound $\W_2(\tilde{\mu}_{k-1}, \mu_{\lam_k})$ by $\W_2(\tilde{\mu}_{k-1}, \mu_{\lam_{k-1}})$. Using the triangle inequality for $\W_2$, we have 
\begin{align*}
\W_2(\tilde{\mu}_{k-1}, \mu_{\lam_k}) \leq &\W_2(\tilde{\mu}_{k-1}, \mu_{\lam_{k-1}}) + \W_2(\mu_{\lam_{k-1}}, \mu^*) \\
&+ \W_2(\mu_{\lam_k}, \mu^*)
\end{align*}

In ~\cite{brosse2017sampling}, the authors showed a bound for $\|\mu_{\lam} - \mu^*\|_{\TV}$ in terms of $\lambda > 0$, and it is easy to extend their proof to obtain a bound for $\W_2(\mu_{\lam}, \mu^*)$ (see Lemma~\ref{lem:W2-constraint-conv} and its proof in Appendix~\ref{sec:smooth-convex-set}). 

In order to prove our result, we make the same assumptions on the constraint set $\Omega$ as in ~\cite{brosse2017sampling}:

\begin{assumption}\label{assumption:constraint}
There exist $r, R, \Delta_1 > 0$ such that
\begin{enumerate}
\item $B(0,r) \subset \Omega \subset B(0,D)$ where $B(0,r_0) = \{y \in \R^d: \|x - y\|_2 \leq r_0 \} \ \forall r_0 > 0$,
\item $e^{\inf_{\Omega^c}(f) - \max_\Omega(f)} \geq \Delta_1$, where $\Omega^c = \R^d \textbackslash \Omega$.
\end{enumerate}
\end{assumption}

\begin{lem}\label{lem:W2-constraint-conv}
Let $\Omega \subset \R^d$ satisfy Assumption~\ref{assumption:constraint}. Then $\forall \lam < \frac{r^2}{8d^2}$,
\begin{equation}
\W_2^2(\mu_\lam, \mu^*) \leq C_\Omega^2 d \sqrt{\lam} 
\end{equation}
for some scalar $C_\Omega > 0$ depending on $D, r$ and $\Delta_1$.
\end{lem}

The proof of the previous Lemma is given in Appendix~\ref{sec:smooth-convex-set}. Using these results, the convergence proof is then very similar as for DL-ULA, and is summarized in Theorem~\ref{thm:convergence_DL_MYULA}, whose proof can be found in Appendix~\ref{sec:convergence-constrained}.

\begin{thm} \label{thm:convergence_DL_MYULA} \textbf{\emph{(iteration complexity of DL-MYULA)}}
Let $\Omega \subset \R^d$ be a convex set satisfying Assumption~\ref{assumption:constraint} and $\mu^*$  be a log-concave distribution given by ~\eqref{eq:constrained-dist} where $f$ has $L$-Lipschitz continuous gradient. For every $k \geq 1$, let
\begin{align}
\lam_k = \frac{1}{\frac{8d^2}{r^2} + de^{2k}} % \approx_{\b,\s} \frac{e^{\frac{k}{2s}}}{\W_2(\ol{\mu}_0,\mu^*)^{\frac{1}{s}}},
\end{align}
\begin{align}
n_k = Ld k^2e^{5k} % \approx_{\b,\s} \frac{d  e^{k(\frac{1}{2s}+3)} }{\W_2(\ol{\mu}_0,\mu^*)^{\frac{1}{s}+6}} ,
\end{align}
\begin{align}
\g_k = \frac{1}{Ld} e^{-4k} %\approx_{\b,\s} \frac{\W_2(\ol{\mu}_0,\mu^*)^{\frac{1}{s}+4}}{d e^{k(\frac{1}{2s}+2 )}},
\end{align}
\begin{align}
\tau_k = Dk % \gtrsim_{\b,\s}  \max\l(   \log^2\l( \frac{1}{\epsilon}\r), 1 \r),
\label{eq:thresh-req-thm}
\end{align}
for every $k\ge 1$.
% Above, the subscript $\b,\s$ suppresses the dependence on $\b,\s$ for clarity, with the exact expressions  deferred to the proof. 
%Suppose also that $\tau$ is sufficiently large, as specified in (\ref{eq:assump-on-R}). 
%\log(\frac{d^{\frac{2\alpha}{1+4s}}}{\epsilon^2})
Then, $\forall \epsilon > 0$, we have:
\begin{itemize}
\item After  $N^{\TV} = \mathcal{O}\left(d^{3.5} \epsilon^{-5} \right)$ total iterations, we obtain $\|\hat{\mu}_K - \mu^*\|_{\TV} \leq \epsilon$.
\item After $N^{\W_2} = \tilde{\mathcal{O}}\left(d^{3.5} \epsilon^{-10} \right)$ total iterations, we obtain $\W_2(\hat{\mu}_K, \mu^*) \lesssim \epsilon$. 
\end{itemize}
\end{thm}

We make a few comments about this convergence result.

\paragraph{Smoothness of $\mu_{\lam_k}$} One can notice that outer iterations in DL-MYULA are longer than in DL-ULA. It is easy to see that the Lipschitz constant associated with the penalized distribution $\mu_\lam$ grows as $\mathcal{O}\l(\frac{1}{\lam} \r)$ as $\lam$ goes to $0$.

As $k$ increases and $\lam_k$ decreases, $\mu_{\lam_k}$ becomes less and less smooth.  Thus, for ULA to succeed in approximating $\mu_{\lam_k}$, the step size $\gamma_k$ of ULA iterations reduces accordingly, and the number of iterations increases. 

The choice for $\lam_k$ ensures that $\lam_k < \frac{r^2}{8d^2}$ as required for Lemma~\ref{lem:W2-constraint-conv} to be applicable.

%\paragraph{Decaying penalty} As stated previously, our convergence result allows for using a decaying penalty parameter, instead of a fixed one as required in ~\cite{brosse2017sampling}. Since the choice of $\lam$ impacts the smoothness of the distribution, 
\paragraph{Convergence rate comparison} Table~\ref{table:constrained} summarizes convergence rates in $\TV$ distance for various first-order constrained sampling algorithms. We can see that DL-MYULA outperforms existing approaches, both terms of dimension and accuracy dependences.

\begin{table}[!h]
\centering
\begin{tabular}{|l||*{3}{c|}}\hline
%\backslashbox{Mask}{Decoder}
\makebox[5em]{\small Algorithm} & \makebox[5em]{\small TV} &  \makebox[5em]{\small \makecell{Literature}} \\\hline \hline
PLMC  & \small $d^{12} \wt{O} \l(\epsilon^{-12} \r)$ & \cite{bubeck2018sampling} \\\hline
MYULA & \small $d^{5} \wt{O} \l(\epsilon^{-6} \r)$  &\cite{brosse2017sampling}  \\\hline
DL-MYULA & \small $d^{3.5} \wt{O} \l(\epsilon^{-5} \r)$ & Our work \\\hline
\end{tabular}
\caption{Upper bounds on the number of iterations required in order to guarantee an error smaller than $\epsilon$ in $\TV$ distance for various constrained sampling algorithms.}
\label{table:constrained}
\end{table}

%\anote{single loop?}
